Voting Behaviour and Power in Online Democracy: A Study of LiquidFeedback in Germany's Pirate Party

In recent years, political parties have adopted Online Delegative Democracy platforms such as LiquidFeedback to organise themselves and their political agendas via a grassroots approach. A common objection against the use of these platforms is the delegation system, where a user can delegate his vote to another user, giving rise to so-called super-voters, i.e. powerful users who receive many delegations. It has been asserted in the past that the presence of these super-voters undermines the democratic process, and therefore delegative democracy should be avoided. In this paper, we look at the emergence of super-voters in the largest delegative online democracy platform worldwide, operated by Germany's Pirate Party. We investigate the distribution of power within the party systematically, study whether super-voters exist, and explore the influence they have on the outcome of votings conducted online. While we find that the theoretical power of super-voters is indeed high, we also observe that they use their power wisely. Super-voters do not fully act on their power to change the outcome of votes, but they vote in favour of proposals with the majority of voters in many cases thereby exhibiting a stabilising effect on the system. We use these findings to present a novel class of power indices that considers observed voting biases and gives significantly better predictions than state-of-the-art measures.

==> cpimg <==
UNUSED -- use the version in ../

#! /bin/sh
#
# Copy an image from SRC to DST, transforming it along the way such that
# it is suitable to be used in Latex. 
#
# INVOCATION
#
#   $0 SRC DST
#
# SEE ALSO
# 
#   This code is based on the file "mkimg" in svn/kunegis/papers/phd/. 
#

set -e

if [ -z "$1" -o -z "$2" ] ; then
    echo >&2 "*** Filenames missing"
    exit 1
fi

src="$1"
dst="$2"

# Threshold filesize for converting a file to bitmap 
FILESIZE_THRESHOLD=500000 

if echo "$src" | grep -qE '\.eps$' ; then

    if echo "$dst" | grep -qE '\.pdf$' ; then
	if [ "$(stat -c %s $src)" -lt $FILESIZE_THRESHOLD ] ; then
  	    epstopdf $src --outfile=$dst
	else
	    convert $src -resize 100% $dst
	fi
    else
	echo >&2 "*** Unknown destination file type:  $dst"
	exit 1
    fi

else
    echo >&2 "*** Unknown source file type:  $src"
    exit 1
fi

exit 0


==> texdep <==
UNUSED -- use the version in ../

#! /bin/sh
#
# Determine the dependencies of a *.tex file. 
#
# INVOCATION
# 	$0 FILENAME
#
# OUTPUT
#	List of dependencies, one file per line
#

file="$1"

[ "$file" ] || {
    echo >&2 '*** Missing filename'
    echo >&2 "Invocation:  $0  FILENAME"
    exit 1
}

echo "$file"

<"$file" sed -re '/\\bibliography\{/!d;s,^.*\{,,;s,\}.*$,,;s/,/\
/g' |
while read name ; do
    echo "$name.bib"
done

<"$file" sed -re '/\\includegraphics.*\{/!d;s,^.*\{,,;s,\}.*$,,' |
while read name ; do
    if [ -z "$name" ] ; then
	continue
    fi
    if echo "$name" | grep -qvE '\.pdf$' ; then
	name="$name.pdf"
    fi
    echo "$name"
done

